Solving the Flowgraphs Case with Eclectic

This paper presents a solution for the Flow Graphs case of the Transformation Tool Contest 2013, using the Eclectic model transformation tool. The solution makes use of several languages of Eclectic, showing how it is possible to combine them to address a non-trivial transformation problem in a concise and modulary way.

==> eptcsdata.tex <==
\providecommand{\firstpage}{43}
\providecommand{\publicationstatus}{Pieter Van Gorp, Louis M. Rose, Christian Krause (Eds.):\\
Sixth Transformation Tool Contest (TTC 2013)\\
EPTCS 135, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.135.6}{10.4204/EPTCS.135.6}}
\pdfoutput=1

